Leveraging Entailment Judgements in Cross-Lingual Summarisation

Synthetically created Cross-Lingual Summarisation (CLS) datasets are prone to include document-summary pairs where the reference summary is unfaithful to the corresponding document as it contains content not supported by the document (i.e., hallucinated content). This low data quality misleads model learning and obscures evaluation results. Automatic ways to assess hallucinations and improve training have been proposed for monolingual summarisation, predominantly in English. For CLS, we propose to use off-the-shelf cross-lingual Natural Language Inference (X-NLI) to evaluate faithfulness of reference and model generated summaries. Then, we study training approaches that are aware of faithfulness issues in the training data and propose an approach that uses unlikelihood loss to teach a model about unfaithful summary sequences. Our results show that it is possible to train CLS models that yield more faithful summaries while maintaining comparable or better informativess.

==> rafe_res/fig_turk.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{turk.png}
    \caption{ Screenshot for human evaluation webpage}
    \label{fig:turk}
\end{figure*}

==> rafe_res/tab_aggrefact.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{1.5pt}
\def\arraystretch{1.5}
\begin{tabular}{lcccccc|cccccccc}
\thickhline
\multirow{2}{*}{Models} & \multicolumn{6}{c|}{XSum Test} & \multicolumn{8}{c}{CNN/DM Test}      \\
% \hline
 ~& \multicolumn{1}{l}{Wang'20} & \multicolumn{1}{l}{Cao'22} & \multicolumn{1}{l}{XSF} & \multicolumn{1}{l}{Goyal'21} & \multicolumn{1}{l}{CLF} & \multicolumn{1}{l}{\textbf{Average}} & \multicolumn{1}{l}{FCC} & \multicolumn{1}{l}{Wang'20} & \multicolumn{1}{l}{SEV} & \multicolumn{1}{l}{PTP} & \multicolumn{1}{l}{FRK} & \multicolumn{1}{l}{Goyal’21} & \multicolumn{1}{l}{CLF} & \multicolumn{1}{l}{\textbf{Average}} \\
\hline
% DAE \\
QuestEval \\
QAFactEval \\
\hline
\multicolumn{15}{c}{ALBERT-Based}\\
\hline
\textsc{Summac}$_\textsc{Conv}^\dagger$  & 70.08 &	69.77 &	70.32 &	56.49 &	72.74 &	67.88 & 92.23 &	76.67 &	85.34 &	82.34 &	75.44 &	25.00 & 66.93 &	71.99

\\
\textsc{Summac}$_\textsc{ZS}^\dagger$   & 63.46 &	48.98 &	55.08 &	37.77 &	58.16 &	52.69 & 83.62 &	75.82 &	85.22 &	87.20 &	72.56 &	4.17 &	74.17 &	68.97

\\
% \textsc{ZeroShot} & 73.80  & 67.24 & 70.44    & 61.58   & 75.65       & 69.74  & 93.72 & \textbf{80.91}   & 88.05   & 88.33   & 76.11       & 25.00   & 69.63       & 74.54  \\
\ours  & \textbf{76.43}  & 67.00 & 73.81    & \textbf{71.76}   & \textbf{78.17}      & \textbf{73.43}  & \textbf{94.97} & 80.25   & \textbf{88.71}   & \textbf{90.29}   & \textbf{79.34}       & 25.00   & 76.34       & \textbf{76.41}  \\
\ours$_\textsc{d2s}$    & 71.19  & 66.89 & \textbf{74.86}    & 61.08   & 75.54       & 69.91  & 94.52 & \textbf{80.52}   & 88.52   & 90.16   & 78.55       & 16.67   & \textbf{76.72}    & 75.09  \\
\ours$_\textsc{s2d}$    & 69.12  & \textbf{71.65} & 69.91    & 71.26   & 72.16       &70.82  & 77.95&	76.36&	85.67&	90.15 &	74.83 &	12.5 &71.72 & 69.88
   \\
\hline
\multicolumn{15}{c}{RoBERTa-Based}  \\
\hline
\textsc{Summac}$_\textsc{Conv}$ \\
\textsc{Summac}$_\textsc{ZS}$\\
% \textsc{ZeroShot} & \textbf{63.22}  & 56.93 & 64.29    & 59.93   & 67.41       & 62.36  & \textbf{90.15} & \textbf{80.93}   & 83.21   & 82.26   & 70.27       & 0.00    & 75.86       & 68.95  \\
\ours  & 60.69  & \textbf{60.53} & 68.52    & \textbf{60.84}   & \textbf{69.67}       & \textbf{64.05}  & 86.92 & 76.43   & 84.30   & 82.65   & \textbf{72.92}       & 0.00    & 76.14       & 68.48  \\
\ours$_\textsc{d2s}$    & 62.67  & 58.08 & \textbf{68.63}    & 58.78   & 63.02       & 62.24  & 87.27 & 77.37   & \textbf{84.64}   & \textbf{83.70}   & 72.01       & 0.00    & \textbf{79.99}       & \textbf{69.28} \\
\ours$_\textsc{s2d}$    & 63.08  & 55.02 & 51.09    & 51.07   & 63.13       & 56.68  & 61.92 & 74.33   & 77.37   & 73.29   & 63.44       & \textbf{12.50}   & 52.14       & 59.28 \\
\thickhline
\end{tabular}
\caption{\label{tab:res_aggrefact}Results on AggreFact. 
For XSum Test, XSF and CLF refer to XSumFaith and CLIFF, respectively. 
PTP, FCC, SEV and FRK refers to Polytope, FactCC, SummEval and FRANK, respectively. 
Numbers with $^\dagger$ are taken from   
\citet{laban-etal-2022-summac}.
}
\end{table*}

==> rafe_res/tab_reduction.tex <==
\begin{table}[t]
\centering
% \small
\setlength{\tabcolsep}{1.5pt}
\def\arraystretch{1.5}
\begin{tabular}{lccc}
\thickhline
Models & \multicolumn{1}{l}{R-L} & \multicolumn{1}{l}{NLI} & \multicolumn{1}{l}{Human}\\
\hline
DAE \\
\textsc{SummaC}$_\textsc{Conv}$ \\
\ours~(w/o rewriting) \\
\ours \\
\thickhline
\end{tabular}
\caption{\label{tab:train}Summarization performance with varied methods for faithfulness estimation. }
\end{table}

==> rafe_res/tab_score.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{1.5pt}
\def\arraystretch{1.5}
\begin{tabular}{lccc}
\thickhline
Models & \multicolumn{1}{l}{AggreFact$_\textsc{xs}$} & \multicolumn{1}{l}{AggreFact$_\textsc{cd}$} & \multicolumn{1}{l}{Summac}\\
\hline
Conv \\
~~~~$p_e$ \\
~~~~$p_e-p_c$ & 70.16 & 72.04 & 77.80\\
ZS \\
~~~~$p_e$ & 69.74 & 74.54  \\
~~~~$p_e-p_c$ & 56.60 & 69.03 & 74.32 \\
\ours \\
~~~~$p_e$ & 74.58 & 68.48 & 82.62\\
~~~~$p_e-p_c$ \\
\thickhline
\end{tabular}
\caption{
\label{tab:score}
Performance change of subtracting the probability of contradiction for varied faithfulness estimators. XS and CD references to the XSum and CNN/DM subsets, respectively.
\yumo{may be good to make this a bar chart}}
\end{table}

==> rafe_res/tab_summ_faithful.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\def\arraystretch{1.2}
{
\footnotesize
  \begin{tabular}{@{}c@{\hspace{0.4cm}}l@{\hspace{0.2cm}}|c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}@{}}
  \hline
& Model & RL & LaBSE & \ours &  UniEval \\
\hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=m]{90}{fr-en}}}

& Vanilla   & 32.71 & 67.11& 48.95 & 56.99  \\
& Random    & 32.02 &65.07& 47.22 & 56.97\\
\cdashline{2-6}
&    Clean     & 32.93 &67.54 & 58.63 & 59.02  \\
&   Mask     & 32.92 &67.55 &\textbf{59.34} &59.34 \\
& Unlike$_{PR}$ & \textbf{33.49} &\textbf{67.61} & 57.49   &\textbf{59.40}       \\
\hline

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=m]{90}{de-en}}}
& Vanilla    & 34.28 &67.58 & 50.73 &59.29 \\
& Random    &33.92 &64.27 &50.21 &56.27 \\
\cdashline{2-6}
& Clean      & 34.09 &67.69 & 51.94&58.54 \\
& Mask       & 34.50 &68.23 & \textbf{55.01}  &\textbf{60.65}   \\
& Unlike$_{PR}$     & \textbf{34.63}  &\textbf{68.26}&  54.19 &60.62  \\
\hline

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=m]{90}{zh-en}}}
& Vanilla     & 33.49 &67.98& 55.23&57.30  \\
& Random    & 33.02&64.24&53.92& 55.36\\
\cdashline{2-6}
& Clean     &33.59&68.03&54.56&57.18  \\
& Mask      &33.45  &68.04& 57.43  & \textbf{58.18}   \\
& Unlike$_{PR}$    & \textbf{33.87} &\textbf{68.86}& \textbf{58.77} & 57.25      \\
\hline

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=m]{90}{cs-en}}}
& Vanilla    & 34.47 &69.01& 48.51&60.04  \\
& Random    & 33.25 &66.41&48.06&58.12\\
\cdashline{2-6}
& Clean     &34.45  &69.07&49.05 &59.81 \\
& Mask      & 34.50 &69.15&49.93  & 59.78   \\
& Unlike$_{PR}$ & \textbf{34.89} &\textbf{69.54}& \textbf{50.74}   & \textbf{61.89}     \\
\hline
  \end{tabular}  
 }
\caption{Results on the Test$_{Faith}$ splits derived from test sets in XWikis.
Average \ours, ROUGE-L (RL), LaBSE, and UniEval.
}
\label{tab:faithful:results}
\end{table} 


==> rafe_res/tab_summ_results.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\def\arraystretch{1.2}
{
\footnotesize
  \begin{tabular}{@{}c@{\hspace{0.4cm}}l@{\hspace{0.2cm}}|c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}@{}}
  \hline
& Model & RL & LaBSE & \ours &  UniEval \\
\hline

\parbox[t]{4mm}{\multirow{5}{*}{\rotatebox[origin=m]{90}{fr-en}}}
& Vanilla   & 31.33 & 64.95& 38.14 & 55.17  \\
& Random    & 31.09 & 63.00&40.96 & 55.08\\
\cdashline{2-6}
& Clean      & 31.27 &65.20 &46.70 &56.86 \\
%& Truncate        \\
& Mask        & 31.23 &65.11 & \textbf{47.54} & 56.69  \\
%& Unlike &  31.37&64.22	&48.30& 56.77      \\
& Unlike$_{PR}$ & \textbf{31.55} &\textbf{65.35} & 46.49   &\textbf{57.21}      \\
\hline


\parbox[t]{4mm}{\multirow{5}{*}{\rotatebox[origin=m]{90}{de-en}}}
& Vanilla    & 32.15 &66.21 & 41.73 &57.60  \\
& Random     &32.01  & 64.23&41.28  &56.47  \\
\cdashline{2-6}
& Clean      & 32.04 &66.21 & 43.11&58.26 \\
% 35.49
% 12.56
% 32.01

%& Truncate        \\
& Mask       & 32.23 & 66.53 & \textbf{45.68}  &58.35   \\
% & Unlike &  32.20&	65.14&44.53 &57.33    \\
& Unlike$_{PR}$     & \textbf{32.31}  &\textbf{66.65}&  44.45 &\textbf{58.61}  \\
\hline


\parbox[t]{4mm}{\multirow{5}{*}{\rotatebox[origin=m]{90}{zh-en}}}
& Vanilla     & \textbf{31.57} &64.37& 43.91&53.21  \\
& Random &30.43  &61.97 &43.11 &52.92 \\
\cdashline{2-6}
& Clean     &31.46&64.30&44.07&53.36  \\
% 34.78
% 12.08
% 30.43

%& Truncate    &  & &     \\
& Mask      &31.36  &64.08& 47.85  & \textbf{54.39}   \\
% & Unlike &  31.09 &63.90&49.03 & 53.10    \\
& Unlike$_{PR}$    & 31.48 &\textbf{64.52}& \textbf{49.22} & 53.91     \\
\hline

\parbox[t]{2.8mm}{\multirow{5}{*}{\rotatebox[origin=m]{90}{cs-en}}}
& Vanilla    & \textbf{32.94} &67.33& 37.53&57.51  \\
& Random & 31.81 &64.82 & 37.36  & 57.19     \\
\cdashline{2-6}
& Clean     &32.82  &67.27&39.26 &57.69  \\
%& Truncate        \\
& Mask      & 32.70 &67.24&39.04  & 57.45   \\
% & Unlike & 32.03&65.78&	40.10  &57.65   \\
& Unlike$_{PR}$ & 32.65 &\textbf{67.39}& \textbf{41.30}   & \textbf{58.55}    \\
\hline



  \end{tabular}  
 }
 \vspace{-0.2cm}
\caption{Results on the XWikis test splits.
Average \ours, ROUGE-L (RL), LaBSE, and UniEval scores. 
}
\label{tab:comparative:results}
\end{table} 


==> rafe_res/tab_summac.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{1.1pt}
\def\arraystretch{1.5}
\begin{tabular}{lccccccc}
\thickhline
Models & \multicolumn{1}{l}{CGS} & \multicolumn{1}{l}{XSF} & \multicolumn{1}{l}{PTP} & \multicolumn{1}{l}{FCC} & \multicolumn{1}{l}{SEV} & \multicolumn{1}{l}{FRK} & \multicolumn{1}{l}{\textbf{Average}} \\
\hline
% NER-Overlap &53.00 &63.30 &52.00 &55.00 &56.80 &60.90 &56.80\\
DAE &63.4 &50.80 &62.80 &75.90 &70.30 &61.70 &64.20 \\
QuestEval &62.60 &62.10 &70.30 &66.60 &72.50 &82.10 &69.40 \\
% MNLI-doc &57.60 &57.50 &61.00 &61.30 &66.60 &63.60 &61.30 \\
\hline
\multicolumn{8}{c}{ALBERT-Based}\\
\hline
\textsc{Summac}$_\textsc{Conv}^\dagger$  & 67.60 & 70.20 & 62.40 & 92.20    & 86.00   & 88.40   & 77.80     \\
\textsc{Summac}$_\textsc{ZS}^\dagger$  & 73.10 & 58.00   & 60.30 & 83.70    & 85.50 & 85.30   & 74.32    \\
% \textsc{ZeroShot} \\
\ours & \textbf{83.77} & \textbf{75.14} & 63.52     & \textbf{94.94}   & 88.70     & \textbf{89.65} & 82.62    \\
\ours$_\textsc{d2s}$   & 83.65 & 74.97 & \textbf{64.86}     & 94.49   & \textbf{88.90}     & 89.39  & \textbf{82.71}    \\
\ours$_\textsc{s2d}$   & 68.35 & 63.87 & 62.95     & 71.71   & 83.05     & 86.71  & 72.78    \\
\hline
\multicolumn{8}{c}{RoBERTa-Based} \\
\hline
\textsc{Summac}$_\textsc{Conv}$\\
\textsc{Summac}$_\textsc{ZS}$ \\
% \textsc{ZeroShot}    & 76.12 & 64.59 & 59.27     & 90.15   & 83.38     & 84.58  & 76.35    \\
\ours  & 80.16 & \textbf{68.37} & 62.61     & 87.27   & 84.49     & \textbf{82.16}  & 77.51    \\
\ours$_\textsc{d2s}$    & \textbf{81.34} & 66.87 & \textbf{64.29}     & \textbf{87.31}   & \textbf{84.86}     & 81.85  & \textbf{77.75}    \\
\ours$_\textsc{s2d}$    & 63.94 & 54.51 & 61.66     & 62.03   & 78.54     & 78.03  & 66.45   \\
\thickhline
\end{tabular}
\caption{\label{tab:res_summac}Results on SummaC. 
PTP, FCC, SEV and FRK refers to Polytope, FactCC, SummEval and FRANK, respectively. 
Numbers with $^\dagger$ are taken from 
\citet{laban-etal-2022-summac}.
}
\end{table}

==> rebuttal_rich.tex <==
# rebuttal

## **R1 m5FT**

We greatly appreciate the thoughtful and constructive feedback provided in your review. 

### **Summary Of Weaknesses:**

- **Weakness**: The paper only focuses on experiments within the XNLI setup, though I think it should compare this to other monolingual-based approaches (e.g. using machine translation).
    
    **Response:**
    
    Thank you for your insightful comments regarding the scope of our experimental comparison. In our paper, we indeed focus primarily on the XNLI setup to evaluate the performance of our models in cross-lingual summarization. In Table 9, we present a thorough analysis within a monolingual (specifically English) context. This section employs INFUSE as a representative NLI evaluator, UniEval as a representative QA evaluator, and LaBSE as a representative cosine similarity evaluator, showcasing our approach’s consistency and reliability in monolingual settings as well.
    
    Regarding the integration of machine translation as a comparative baseline, we carefully considered this option. However, we identified several potential complications that could affect the purity and interpretability of our results. Notably, machine translation systems may introduce additional variables such as hallucination. These errors pose significant challenges in attributing observed performance changes—whether they stem from the inherent capabilities of the model or from artifacts introduced by the translation process itself.
    
    Given these considerations, we aimed to minimize external dependencies and potential confounders in our experimental design to provide a clear and focused evaluation of the capability of different approaches.
    
- **Weakness**: With rapid development of LLMs and its successful application on abstractive summarization, I'm not sure how much of this improved modeling techniques can be applied towards LLM-based summarization systems.
    
    **Response:**
    
    We acknowledge your concern regarding the applicability of our faithfulness-aware training techniques to LLM-based summarization systems amid their rapid development. In this paper, we first validate the effectiveness of the multi-lingual NLI model, ensuring it can be used to detect unfaithful summaries in training data of cross-lingual settings. Then, we study training approaches that are aware of unfaithfulness sentences. From these two aspects,  
    
    (1) By integrating the NLI model as a component in LLM-based summarization systems, we can more accurately filter out or correct unfaithful elements in the training data. This process not only improves the quality of the generated summaries but also ensures that the system is more robust across different languages, enhancing its applicability and effectiveness in global, multilingual contexts.
    (2) By implementing our unlikelihood loss that is sensitized to the nuances of unfaithful sentences, LLMs can be conditioned to avoid generating such content in their outputs. This approach directly translates to an improvement in the quality of abstractive summarization, ensuring that generated summaries are both relevant and trustworthy.
    
- **Weakness**: This paper haven't referenced a similar work that has been published on using NLI to improve coverage while maintaining factuality https://arxiv.org/pdf/2301.10483.pdf
    
    **Response:**
    
    We acknowledge the oversight of not referencing the work. And we will include this work in the revision. 
    

### **Comments, Suggestions And Typos:**

- I assume the bulk of this work was done before wide adoption of LLMs since the middle of 2023. An important future work would be thinking about ways to apply these methods towards LLM-based systems to improve actuality.
    
    **Response:**
    
    We greatly appreciate your suggestion regarding how to integrate our method in LLM. We will include a dedicated section in the revision of our paper that discusses potential pathways for applying our methods to LLM-based systems.
    

# R2 rMs1

We greatly appreciate the thoughtful and constructive feedback provided in your review. We are grateful to address the insightful points raised.

### **Summary Of Weaknesses:**

- **Weakness**: This paper sounds like stacking existing methods in a straightforward way. Hence, the novelty is low.
    
    **Response:**
    
    Thank you for your review and the opportunity to clarify the innovative aspects of our work. While our research leverages existing methods, the novelty of our approach lies in the strategic selection, modification, and application of these methods to address specific challenges in cross-lingual summarization, particularly in assessing and ensuring the faithfulness of summaries.
    
    **Selection of Methods:** Our research goes beyond merely 'stacking' existing methods. We conducted a comprehensive analysis to determine the most effective NLI inference strategies for our specific context. This meticulous selection process is evidenced by our demonstration that the INFUSE method, among others we tested (FULLDOC, summac, SENTLI), is optimally suited for evaluating the faithfulness of long-text and abstractive summaries, as detailed in Table 2 of our paper.
    
    **Innovative Modification of Existing Techniques:** Recognizing the limitations of direct unlikelihood loss application in language modeling, we innovatively introduced an extra segment embedding to mitigate potential negative impacts. This modification represents an advancement in employing unlikelihood loss for training language models, particularly in preserving informativeness while enhancing content faithfulness.
    
    **Comprehensive Evaluation:** To ensure robust evaluation beyond NLI-based assessments, we incorporated complementary metrics using LaBSE for cosine similarity evaluation and UniEval for QA-based assessment. This comprehensive evaluation framework, tailored for cross-lingual settings, allows us to validate the effectiveness of our approach without relying solely on the NLI model, thereby avoiding circular validation.
    
    By thoughtfully selecting, modifying, integrating, and evaluating these methods, we have developed a faithfulness-aware training approach that prioritizes both informativeness and faithfulness.
    
    We appreciate your feedback and hope this explanation addresses your concerns regarding the novelty and value of our research.
    
- **Weakness**: It is unclear how XNLI is used to improve faithfulness in summarizaiton under cross-lingual settings. XNLI is a pair-wise, cross-lingual NLI dataset.
    
    **Response:**
    
    We apologize for any confusion caused regarding the use of XNLI/X-NLI in our work. X-NLI, as you correctly mentioned, is indeed a NLI dataset designed for evaluating model performance on pair-wise text inference across multiple languages. XNLI refers to cross-lingual NLI in our paper. We leverage the signal from the cross-lingual NLI model to better train the model. Thanks for your notification and we will use cross-lingual NLI instead of XNLI in our revision. 
    
- **Weakness**: It is unclear how the authors computed scores in Table 2. Did they use a model find-tuned on XNLI to measure the entailment score between two sentences in two different languages?
    
    **Response:**
    
    Yes. The backbone NLI model we used was fine-tuned in multilingual setting (French premise/hypothesis or German premise/hypothesis), but never seen cross-lingual samples (French premise with German hypothesis). Thus, we first validate its performance in cross-lingual setting in Table 1. We found that the model shows good performance in cross-lingual settings, so further apply them to assess the faithfulness of the summaries in XWikis in Table 2.   
    
- **Weakness**: An important baseline missing is to translate text pairs into English and then use English only faithfulness metrics.
    
    **Response:**
    
    Thank you for your thoughtful review and suggestion regarding the inclusion of a baseline that involves translating generated summaries into English then applying English-only faithfulness metrics. Your point raises an important consideration in the evaluation of cross-lingual summarization systems.
    
    (1) It's worth noting that previous work, as detailed in the XWikis paper, has explored the pipeline approach of translation followed by summarization and found that it generally underperforms relative to end-to-end methods by approximately 1.5 RougeL points. This finding aligns with our decision to focus on direct cross-lingual approaches rather than employing an intermediary translation step, which, as the XWikis paper suggests, may compromise the overall performance of the summarization.
    
    (2) Furthermore, our research interest extends to the analysis of hallucinations within the pipeline method, which introduces additional complexity. Hallucinations can originate from both the summarization and translation stages, complicating the attribution of errors and potentially reducing faithfulness scores. The integration of a pipeline method would necessitate dividing our research focus between these two distinct processes, making it challenging to ascertain the origin of hallucinations—whether they stem from the summarization model or translation tools. Given the limited scope of this short paper, our primary objective has been to explore training end-to-end summarizers that are both informative and faithful in a cross-lingual setting.
    
    (3) Regarding concerns about our method's performance in an English setting, we have included results for monolingual English in Table 9 to demonstrate the applicability and robustness of our approach across languages, including within a monolingual context.
    
    We acknowledge the value of the suggested pipeline baseline as a potential avenue for future research. As such, we are committed to extending our research in these directions in future work, potentially through a more detailed journal article that could offer a broader and more inclusive exploration of cross-lingual summarization training techniques.
    

### **Comments, Suggestions And Typos:**

- Why sometimes XNLI and other times X-NLI?
Why part of the experiments on mT5 and the others on mBART?
Why cz row and column are missing in Table 1?
Will the authors release their annotations?
Many sentences are unfinished.
    
    **Response:**
    
    (1) Thank you for pointing out the inconsistency in our terminology. As clarified, "X-NLI" refers to the multilingual Natural Language Inference dataset, and "XNLI" denotes cross-lingual NLI specifically. To avoid any confusion in future references,  we will use cross-lingual NLI instead of XNLI in our revision. 
    
    (2) Thank you for raising this question regarding our model selection for the experiments. Our decision to employ mBART for summarization tasks was directly influenced by its prominent use in prior work within the XWikis dataset, ensuring consistency with established benchmarks and methodologies in the field. 
    
    Conversely, the absence of a readily available mBART model fine-tuned for cross-lingual NLI tasks necessitated the adoption of an alternative model for this aspect of our study. We opted for the mT5 model. Prior to its application, we rigorously validated the performance of mT5 in cross-lingual settings, as detailed in Table 1, to ensure its suitability and reliability for our analysis.
    
    An additional advantage of utilizing distinct models for summarization and evaluation is the mitigation of preference bias—a phenomenon where model-based evaluators demonstrate a bias toward summaries generated by the same underlying model. This issue is well-documented in the literature, with studies [1,2] indicating that such bias can compromise the impartiality and trustworthiness of evaluation metrics. By employing mT5 for evaluation and mBART for summarization, we inherently reduce the risk of preference bias influencing our results, thereby enhancing the credibility and objectivity of our evaluative conclusions.
    
    (3) Regarding the absence of Czech (cz) language results in Table 1, we realize this might have been unclear to readers. As detailed in Appendix A (line 648), Czech is not part of the X-NLI test set, limiting our ability to conduct a evaluation for this language. We acknowledge the oversight in not making this explicit in the main text and will amend the manuscript to clearly state the reason for the omission of Czech language results.
    
    (4) Yes, we will release all data, annotation, and code. 
    
    Reference
    
    [1] Understanding factual errors in summarization: Errors, summarizers, datasets, error detectors
    
    [2] Revisiting the gold standard: Grounding summarization evaluation with robust human evaluation.
    

## **R3 bF5n**

We greatly appreciate the thoughtful and constructive feedback provided in your review. We are grateful to address the insightful points raised.

### **Summary Of Weaknesses:**

- **Weakness**: Lack of ablation studies. While their unlikelihood loss that is augmented with additional embeddings yields strong performance, there is no ablation study investigating the effect of the additional embeddings. The additional embeddings can also be used with the normal cross-entropy loss to see whether the unlikelihood loss better leverage the embeddings.
    
    **Response:**
    
    We appreciate the emphasis on the importance of ablation studies to delineate the contributions of different components of our proposed method. Our approach, which integrates unlikelihood loss with additional segment embeddings, was developed with the specific goal of refining the model's language modelling in generated summaries.
    
    The rationale behind introducing additional segment embeddings is to mitigate the potential over-penalization inherent in the direct application of unlikelihood loss. For instance, in the case of an unfaithful phrase like 'New York,' while the generation of 'New' following previous tokens should be penalized to avoid unfaithfulness, the subsequent generation of 'York' given 'New'  should not be similarly penalized to preserve language fluency.
    
    In our preliminary experiments:
    
    - Applying unlikelihood loss without the segment embeddings across all language directions resulted in a noticeable decrease in performance, specifically an average reduction of 0.9 RougeL points compared to the baseline (vanilla model). This underscores the necessity of segment embeddings in counterbalancing the stringent nature of unlikelihood loss.
    - Furthermore, we tested the application of mask loss with segment embeddings in German (de) and French (fr) language settings. These trials indicated no significant change in performance, suggesting that the beneficial effects observed are specifically attributable to the synergistic combination of unlikelihood loss and segment embeddings, rather than the segment embeddings alone.
    
    Acknowledging the critical insight provided by your review, we realize the necessity of including a detailed ablation study to explore and articulate the distinct impact of the additional segment embeddings within our framework. We will incorporate a comprehensive ablation section in the final version of our manuscript. This section will detail the intuition behind our methodological choices, and present the outcomes of our preliminary experiments.
    
- **Weakness**: No human evaluation. They only present results with automatic metrics, while they could produce inaccurate evaluation.
    
    **Response:**
    
    Thank you for your constructive feedback regarding the evaluation of our model-generated summaries. We understand the importance of human evaluation in assessing the faithfulness and informativeness of summaries, especially in light of the limitations associated with automatic evaluation metrics, which may not fully capture human judgment.
    
    However, our research setting poses unique challenges that impact our ability to conduct extensive human evaluations. Specifically, our focus on cross-lingual summarization necessitates the involvement of bilingual annotators who are proficient in both the source and target languages. This requirement significantly narrows the pool of potential annotators, making the process of obtaining high-quality, bilingual annotation both challenging and costly.
    
    The scarcity of such bilingual annotators, combined with the financial constraints, limited our ability to include human evaluation in our study. Despite this, we made concerted efforts to ensure the reliability of our results through the use of three advanced automatic evaluation metrics, LaBSE, INFUSE and UniEval. These metrics, while not perfect, have been validated as reasonably effective in assessing faithfulness and informativeness of summary quality.
    

# **Weakness**:

- 'Considering that the faithfulness evaluation is actually done in the monolingual setting using the provided English documents, it is also unclear why the authors specifically choose UniEval as their faithfulness metric, while there are many other metrics (e.g., QAFactEval).’
    
    **Response:**
    
    No. We use crosslingual setting for LaBSE and INFUSE, and mono-lingual for UniEval.  We select 
    We need a QA based method to avoid using NLI model to evaluate itself.
    uni-eval showed a good correlation with humans in SummEval.
    
    we will include the experiment with QAFactEval. 
    

## **R4 ta3q**

We greatly appreciate the thoughtful and constructive feedback provided in your review. We are grateful to address the insightful points raised.

### **Summary Of Weaknesses:**

- **Weakness**:  No human evaluation of model-generated summaries in terms of faithfulness and informativeness. Although automatic evaluation metrics are used, they still can not fully reflect human opinions. This raises the concern of the reliability of the results reported in the paper.
    
    **Response:**
    
    Thank you for your constructive feedback regarding the evaluation of our model-generated summaries. We understand the importance of human evaluation in assessing the faithfulness and informativeness of summaries, especially in light of the limitations associated with automatic evaluation metrics, which may not fully capture human judgment.
    
    However, our research setting poses unique challenges that impact our ability to conduct extensive human evaluations. Specifically, our focus on cross-lingual summarization necessitates the involvement of bilingual annotators who are proficient in both the source and target languages. This requirement significantly narrows the pool of potential annotators, making the process of obtaining high-quality, bilingual annotation both challenging and costly.
    
    The scarcity of such bilingual annotators, combined with the financial constraints, limited our ability to include human evaluation in our study. Despite this, we made concerted efforts to ensure the reliability of our results through the use of three advanced automatic evaluation metrics, LaBSE, INFUSE and UniEval. These metrics, while not perfect, have been validated as reasonably effective in assessing faithfulness and informativeness of summary quality.
    
- **Weakness**: The generalizability of the proposed method is not validated, as the experiments are conducted on a single model (mT5-large) on a single dataset.
    
    **Response:**
    
    Thank you for your comment regarding the generalizability of our proposed method. We acknowledge that the scope of our experimental validation, as presented in the paper, is focused primarily on the mBART model and the XWikis dataset. This decision was influenced by several factors, which we outline below:
    
    1. **Resource Constraints:** As a short paper, we faced inherent limitations in the scope and scale of the experiments we could conduct. These constraints extended to computational resources, which influenced our decision to concentrate on a single model and dataset. Despite these limitations, we endeavored to provide a meaningful contribution within the scope of our research.
    2. **Dataset Representativeness:** The XWikis dataset encompasses five language directions, each with around 100k data pairs. This substantial volume and linguistic diversity provide a robust foundation for evaluating our method's efficacy across different languages. We believe that the size and scope of the XWikis dataset contribute significantly to the validity and relevance of our findings, even within the bounds of a single dataset study.
    
    We appreciate the concern for the generalizability of our findings and agree that further validation across additional models and datasets (eg, in other domains) would be valuable. This future work will aim to address the generalizability concerns and further validate the applicability of our approach to a broader array of NLP tasks and settings.
    
- **Weakness**: Lack of novelty. The paper applies existing methodologies in cross-lingual summarization without mentioning difficulties or solutions specific to cross-lingual summarization. Specifically, the NLI model for faithfulness evaluation, and methods to train more faithful summarization models, are all from previous works.
    
    **Response:**
    
    Thank you for your review and the opportunity to clarify the innovative aspects of our work. While our research leverages existing methods, the novelty of our approach lies in the strategic combination, modification, and application of these methods to address specific challenges in cross-lingual summarization, particularly in assessing and ensuring the faithfulness of summaries.
    
    1. **Strategic Combination of Methods:** Our research goes beyond merely 'stacking' existing methods. We conducted a comprehensive analysis to determine the most effective NLI inference strategies for our specific context. This meticulous selection process is evidenced by our demonstration that the INFUSE method, among others we tested (FULLDOC, summac, SENTLI), is optimally suited for evaluating abstractive summary faithfulness, as detailed in Table 2 of our paper.
    2. **Innovative Modification of Existing Techniques:** Recognizing the limitations of direct unlikelihood loss application in language modeling, we innovatively introduced an extra segment embedding to mitigate potential negative impacts. This modification represents an advancement in employing unlikelihood loss for training language models, particularly in preserving informativeness while enhancing content faithfulness.
    3. **Comprehensive Evaluation:** To ensure robust evaluation beyond NLI-based assessments, we incorporated complementary metrics using LaBSE for cosine similarity evaluation and UniEval for QA-based assessment. This comprehensive evaluation framework, tailored for cross-lingual settings, allows us to validate the effectiveness of our approach without relying solely on the NLI model, thereby avoiding circular validation.
    
    By thoughtfully selecting, modifying, integrating and evaluating these methods, we have developed a faithfulness-aware training approach that prioritizes both informativeness and faithfulness.
    
    We appreciate your feedback and hope this explanation addresses your concerns regarding the novelty and value of our research.
    

- **Weakness**: No baseline considered in Section 3.2. More explanations are required if there is no baseline available in the cross-lingual summarization setting.
    
    **Response:**
    
    We appreciate your observation regarding the baseline comparisons in Section 3.2. To clarify, our study does incorporate two baselines to ensure a robust evaluation framework. 
    
    1. **Vanilla:** This baseline represents the standard approach to the task without incorporating any specific mechanisms to enhance faithfulness in the generated summaries. By including this baseline, we aim to provide a foundational comparison point that illustrates the effectiveness of our proposed method against a conventional setup where no additional faithfulness information is provided.
    2. **Clean:** The second baseline, referred to as "clean," involves a preprocessing step where noisy data are directly filtered out from the training set. This approach seeks to improve the quality of the input data and, by extension, the faithfulness of the generated summaries through data curation rather than through the modification of the model architecture or training process.
    

### **Comments, Suggestions And Typos:**

- a. line 111-112 If the model is finetuned on English premise and hypothesis pairs, why can it predict on a cross-lingual setting? Is the mT5-large model already finetuned on premise-hypothesis pairs from different languages?
    
    b. line 127. It would be better to rephrase "we make use of XNLI to assess" as "we make use of a cross-lingual NLI model to assess the faithfulness of summaries in a cross-lingual setting."
    
    c. line 188. What's the purpose of the math formula? The formula is the likelihood of the generated summary, but it is not clear the purpose of putting the formula here.
    
    d. line 195. Please explain more: "these annotations are propagated back to tokens"
    
    e. line 835. How do you decide the value of X for different languages (e.g., 10 for German)?
    
    f. line 213. It would be better to mention that INFUSE gives span-level prediction. Otherwise it can be confusing as NLI model usually gives sentence-level prediction.
    
    g. line 256. It would be better to replace "content adequacy" with "informativeness"
    
    h. Is there any previous work on evaluating and improving faithfulness in cross-lingual summarization? If not, it would be better to mention this point in the introduction.
    
    i. How are the faithfulness labels obtained for the 238 Xwikis samples? (Some human annotation is conducted, or there are already annotations in the original dataset?)
    
    **Response:**
    
    a. The mT5 NLI model is fine-tuned in multilingual settings, eg, seen the French premise/hypothesis and German premise/hypothesis but never seen a cross-lingual sample such as the French premise with German hypothesis.  That's the reason why we need to validate the efficacy of the model before applying it in assessing the faithfulness of summaries.
    
    b.c.h.g We appreciate your careful review and the specific suggestions for improving the clarity and accuracy of our manuscript. We agree with your recommendations and will make the following modifications in the revised version.
    
    d. When a sentence within a summary is identified as unfaithful, this unfaithfulness label is applied to each constituent token of the sentence. 
    
    e. The determination of the value X for different languages was informed by an analysis of average entailment scores obtained from our cross-lingual NLI model across five languages. This inspection revealed lower entailment scores for English and Chinese, suggesting a higher prevalence of unfaithful content in summaries in these languages. Based on these findings, we chose threshold values (e.g., 10 for German, French, and Czech; 20 for Chinese and English) tailored to the observed levels of faithfulness in each language, optimizing our model's sensitivity to unfaithfulness. 
    
    f. INFUSE also produces sentence-level annotation.
    
    i. We email one of the authors and obtain the faithfulness labels. They have also granted permission for these annotations to be published.

==> xfaith_res/sec_nli.tex <==
\subsection{How to evaluate Entailment in Document-Summary Pairs}
In this section, we discuss how to leverage X-NLI models to serve as content adequacy evaluators on CLS task. Following previous work \cite{maynez-etal-2020-faithfulness} \cite{DBLP:journals/tacl/LabanSBH22}, we assume that a summary should be entailed by the document. In other words, the content conveyed by each sentence in a summary should be supported by the corresponding document. 

We can assess entailment between each sentence in a summary and each sentence in the document using the X-NLI models. However, due to the nature of abstractive summarisation, a summary sentence can aggregate information from multiple sentences in a document. In this case, by evaluating one document sentence at a time, entailment will fail for each of the summary sentences. Laban et al.\cite{DBLP:journals/tacl/LabanSBH22} have also taken all document sentences as the premise and evaluated entailment for each sentence in the summary. Thus, we can divide the discussion into different ways we can take sentences from the document (premises) and sentences from the summary (hypothesis) for entailment evaluation. At a high level, we split the discussion into two parts, the one-to-one relationship, and the many-to-one relationship. 


\subsubsection{One-to-One Relationship}

We generate a XNLI sentence pair (premise, hypothesis) by a (document, summary) pair at the sentence level. Specifically, the document is split into sentences, as premises labeled from Doc$_X$ = \{$P_{1},...,P_{M}$\}. 
%$D_{1},...,D_{M}$. same applies for summary S_....
The summary is also split into sentences, as hypotheses labeled from Sum$_Y$ = \{$H_{1},...,H_{N}$\}.

The X-NLI
%NLI-based 
models run over each sentence pair ($P_{m}, H_{n}$) and generate a probability distribution over three labels: entailment, contradiction, and neutral. Laban et al. \cite{DBLP:journals/tacl/LabanSBH22} revealed that using different combinations of three labels only slightly influences the result. For simplicity, we only pick the probability of entailment for the following experiments. After that, we form an $M \times N$ matrix $E$ consisting of the entailment scores $E_{mn}$, where m and n are the indexes of sentences in the document and summary, respectively. 

In the one-to-one relationship, we assume each summary sentence $H_{n}$ is supported by only one document sentence $P_{m}$. Intuitively, for the summary sentence, only the document sentence $P_{m}$ with the top entailment score (the strongest support) should be selected. We apply the max operator on each matrix column and obtain a $1 \times N$ vector. We take the mean operator on the vector to produce the final score for a document-summary pair. 

\subsubsection{Many-to-One Relationship}

In the many-to-one relationship, we assume each summary sentence $H_{n}$ can be supported by more than one document sentence \{${P_{j}, \cdots, P_{k}}$\}. We refer to them as $P_{many}$. The core problem is, \textbf{ how to find $P_{many}$ in the document}, which can correctly entail $H_{n}$. We heuristically propose three strategies to search for such sentences. 


\subsection{others}
Assess content overlap with different ways of applying XNLI (i.e., different ways of taking sentences from the input document) and 
at the sentence and sub-sentence level for summary sentences.
To split long sentences (sub-sentence level) we use sentence 
rewriting. 
Compare with human annotations (those collected 
for dataset validation in \cite{perez-beltrachini-lapata-2021-models,huajian2022}.
An error analysis is provided in \cite{huajian2022}. 
We can also do some study of the limitations of XNLI \cite{durmus-etal-2022-spurious}?
We have seen that 
it works differently for different datasets. It works better for WikiLingua
(simpler, shorter and extractive sentences)
than more complex abstractive datasets XWikis and Voxeurop.

